Multi-Object Navigation in real environments using hybrid policies

Navigation has been classically solved in robotics through the combination of SLAM and planning. More recently, beyond waypoint planning, problems involving significant components of (visual) high-level reasoning have been explored in simulated environments, mostly addressed with large-scale machine learning, in particular RL, offline-RL or imitation learning. These methods require the agent to learn various skills like local planning, mapping objects and querying the learned spatial representations. In contrast to simpler tasks like waypoint planning (PointGoal), for these more complex tasks the current state-of-the-art models have been thoroughly evaluated in simulation but, to our best knowledge, not yet in real environments. In this work we focus on sim2real transfer. We target the challenging Multi-Object Navigation (Multi-ON) task and port it to a physical environment containing real replicas of the originally virtual Multi-ON objects. We introduce a hybrid navigation method, which decomposes the problem into two different skills: (1) waypoint navigation is addressed with classical SLAM combined with a symbolic planner, whereas (2) exploration, semantic mapping and goal retrieval are dealt with deep neural networks trained with a combination of supervised learning and RL. We show the advantages of this approach compared to end-to-end methods both in simulation and a real environment and outperform the SOTA for this task.

==> sota_raw.tex <==
\section{Related work}
\label{sec:sota}
\myParagraph{Modular Embodied Navigation} TO FILL 
- Chaplot (ObjectNav paper~\cite{Chaplot2020Learning} + PONI~\cite{ramakrishnan_poni_2022}) 
- Robot Navigation with Map-Based Deep Reinforcement Learning -  \cite{argo21}
\\

\myParagraph{Sim2Real} TO FILL - Bidirectional Sim2Real \cite{truong21bidirectional} - RobustNav -  Predictivity \cite{kadian_sim2real_2020}
- ICRA22 best paper~\cite{saha22icra} 
\\

\myParagraph{Memory and Maps (Inductive Bias)} TO FILL - Ed (EgoMap)~\cite{BeechingECCV2020}- NeuralMap - Vedaldi (MapNet)
\\

\myParagraph{Exploration} TO FILL - Chaplot (ANL + SemExp) - Chen et al (coverageb based) - Curiosity Paper - Frontier-based exploration paper ??(citation?)
\\


\section{Related work}
\label{sec:sota}
\myParagraph{Modular Embodied Navigation} TO FILL 
- Chaplot (ObjectNav paper~\cite{Chaplot2020Learning} + PONI~\cite{ramakrishnan_poni_2022}) 
- Robot Navigation with Map-Based Deep Reinforcement Learning -  \cite{??}

%learning for exploration is well motivated, 
Casting a task as an end-to-end learning problem is 
%well motivated and 
widely used in CV and NLP communities. %~\cite{Chen19explorat}.
%Chen et al. (2019) has used end-to-end learning to tackle this problem. Their
%motivation is three fold: a) learning provides ﬂexibility to the choice of input modalities (classical
%systems rely on observing geometry through use of specialized sensors, while learning systems can
%infer geometry directly from RGB images), b) use of learning can improve robustness to errors in
%explicit state estimation, and c) learning can effectively leverage structural regularities of the real
%world, leading to more efﬁcient behavior in previously unseen environments. 
For the exploration problem,~\cite{Chen19exploration} designed an end-to-end trained neural network based policy that processed raw sensory observations to directly output actions that the agent should execute.
However, learning all together the mapping, state-estimation and
path-planning purely from data %in an end-to-end manner 
is prohibitively expensive~\cite{Chaplot2020Learning}.
%To address the prohibitive cost, 
Alternative methods~\cite{Chaplot2020Learning,Chaplot20objectgoal,BeechingECCV2020,Chaplot2020semantic} propose hybrid architectures that compose a learned mapper with global and local policies, where all components are interfaced via the map and an analytical path planner. 
%The learned mapper produces free space maps from input RGB images exploit structural regularities in layout of real world environments to produce long-term goals~\cite{Chaplot2020Learning}

%--- PONI ----
Following the modular approach, Ramakrishnan~\etal ~\cite{ramakrishnan_poni_2022} disentangle the skills of ‘where to look?’ for an object and ‘how to navigate to (x, y)?’.
%insight is that ‘where to look?’ task of exploration
% can be treated purely as a
%perception problem, and learned without environment interactions. 
%To address this, we 
Their network predicts two complementary potential functions conditioned on
a semantic map and uses them to decide where to look for an unseen object. 
The %potential function 
network %using supervised learning 
is trained on top-down semantic maps, and integrated into a modular framework to perform ObjectNav. 

\\

\myParagraph{Sim2Real} 

%no simulation is perfect, and robots trained solely in simulation fail to generalize to the real-world, resulting in a “sim-vs-real gap”. How to overcome the trade-off between the abundance of less accurate, artificial data from simulators and the scarcity of reliable, real-world data?

%No simulation can perfectly replicate reality. 
Despite the %tremendous
progress in computer graphics and game engine technology, highly used in robot learning, the sim2real gap can compromise any strong performance achieved in simulation when agents are tested in the real-world~\cite{hofer2020sim2real}. 
%trying to replicate it in reality. 
Perception and control policies learned in simulation often do not generalize well to real robots due to  inaccuracies in modelling, simplifications and biases. To close the gap, domain randomization methods~\cite{tan18real,peng18sim} assume that the real world distribution is a randomized instance of the simulation environment; they treat the discrepancy between the domains as variability in the simulation parameters. 

Alternatively, domain adaptation methods learn an invariant mapping function for matching distributions between the simulator and the robot environment. Related examples to the work presented here include 
%using synthetic objects to learn a vision based grasping model~\cite{grasp}, 
sim2real transfer of visuo-motor policies for goal-directed reaching movement by adversarial learning~\cite{zang19adversarial}, adapting dynamics in reinforcement learning~\cite{eysenbach21off}, and adapting object recognition model in new domains~\cite{zhu19adapting}. 
Kadian~\etal~\cite{kadian_sim2real_2020} 
investigated the sim2real predictivity of Habitat-Sim~\cite{Savva_2019_ICCV} for PointGoal navigation and proposed a new metric to quantify predictivity, called Sim-vs-Real Correlation Coefﬁcient (SRCC).
%and developed a library for seamless transferring simulation-trained agents to a LoCoBot platform with a minimal code change.
Recently, Chattopadhyay~\etal~\cite{chattopadhyay2021robustnav} benchmarked the robustness of embodied agents to visual and dynamics corruptions, finding that agents trained in simulation severely under-perform when evaluated in corrupted target environments. They show that although standard data-augmentation techniques and self-supervised adaptation strategies offer some improvement, much remains to be done in terms of fully recovering lost performance.

Recently,~\cite{truong_bi-directional_2021}, 
%a bi-directional  method adapts the sensor gap from real2sim and the dynamics gap from sim2real.
%Bidirectional Sim2Real~\cite{truong21bidirectional} - 
proposed a bi-directional adaptation layer that bridges the sim2real gap in both directions– real2sim to bridge the visual domain gap, and sim2real to bridge the dynamics domain gap.
%We demonstrate the benefits of BDA on the task of PointGoal Navigation.

%We instantiate and demonstrate the benefits of BDA on the task of PointGoal Navigation (PointNav) [14], which involves an agent navigating in a previously unseen environment from a randomized initial starting location to a goal location specified in relative coordinates. For controlled experimentation, and due to COVID-19 restrictions, we use Sim2Sim transfer of PointNav policies as a stand-in for Sim2Real transfer. We conduct experiments in photo-realistic 3D simulation environments using Habitat-Sim~\cite{habitat-sim}, which prior work~\cite{predictivity} has found to have high sim2real predictivity, meaning that inferences drawn in simulation experiments have a high likelihood of holding in reality on Locobot mobile robot.

The PointGoal task is evaluated on real robots in~\cite{SadekICRA2022}. To reach competitive performance without modelling any sim2real transfer, the agent is pre-trained on a wide variety of tasks and then fine-tuned on a simulated version of the target environment. %, i.e. by deploying the trained agent directly from simulation to a real physical robot. 

\bc{say that moving from PointGoal to more complex tasks add new aspects to sim2real transfer.
Exploration and dynamic mapping, gap between virtual objects and their physical realizations.}
%RobustNav~\cite{chattopadhyay2021robustnav} -
%Predictivity~\cite{kadian_sim2real_2020} -
%ICRA22 best paper~\cite{saha22icra} 
\\


\myParagraph{Memory and Maps (Inductive Bias)} TO FILL - Ed (EgoMap)~\cite{BeechingECCV2020}- NeuralMap - Vedaldi (MapNet)
\\

% mapnet
\cite{henriques18mapnet}
 reasoning about 3D space and geometry, particularly in relation to
large environments

Mapnet propose and study a new distributed representation of 3D environments that can be used
in a deep learning context. The representation is used by a recurrent neural network to interpret an environment
seen through a moving camera. The representation works as a mapping component, i.e. a dynamic spatial memory
which is updated incrementally from the camera observations. This memory allows the recurrent network to remember places visited in the past, as well as to relocalize itself with respect to those.
Our design addresses two challenges. The ﬁrst one is to allow the model to factor egocentric and allocentric information. 


%Neural map
\cite{parisotto18neuralmap}
Memory is a crucial aspect of an intelligent agent’s ability to plan and reason in partially observable
environments.
NeuralMap is a structured memory designed speciﬁcally for reinforcement learning agents in 3D environments. 
%The Neural Map architecture overcomes some of the shortcomings of the previously men-tioned neural memories. 
First, it uses an adaptable write operation and so its size and computational
cost does not grow with the time horizon of the environment as it does with memory networks.
Second, we impose a particular inductive bias on the write operation so that it is 1) well suited
to 3D environments where navigation is a core component of sucessful behaviours, and 2) uses a
sparse write operation that prevents frequent overwriting of memory locations that can occur with
NTMs and DNCs

%Egomap
\cite{BeechingECCV2020}
One example is EgoMap is a spatially structured neural memory architecture. EgoMap
augments a deep reinforcement learning agent’s performance in 3D environments on challenging tasks with multi-step objectives. The EgoMap architecture incorporates several inductive biases including a differentiable inverse projection of CNN feature vectors onto a top-down spatially structured map. The map is updated with ego-motion measurements through a differentiable transform.
It uses projective geometry as an inductive bias to neural networks, allowing
the agent to structure its memory with respect to the loca-
tions of objects it perceives




\myParagraph{Exploration} 
%TO FILL 
%- Chaplot (ANL + SemExp) 
%- Chen et al (coverageb based) 
%- Curiosity Paper 
%- Frontier-based exploration paper 

%The role of exploration in navigation suggests that 
%exploration is itself an important task that can be studied and quantitatively evaluated. For example, an agent can be tasked with exploring a previously unseen environment
%within a path-length budget (maximal trajectory length, at the end of which the exploration episode is terminated).
%One possible measure for evaluating an exploration episode is the coverage of the environment: what fraction of the previously unseen environment the agent has covered during the episode.\cite{anderson18vision}

\cite{Chaplot2020Learning}
%Irrespective of the task or the setting, a core problem in navigation is exploration, i.e., 
Exploration is a core problem in any navigation task. %wherever is the task setting.
Efficiently visiting the environment is useful for solving tasks in known environments and pre-mapping in unknown environments. Due to its importance,
%a role of exploration in navigation suggests,  
exploration itself %an important task that is 
can be studied and quantitatively evaluated~\cite{evaluaion}. 
%For example, an agent can be tasked with exploring a previously unseen environment within a path-length budget (maximal trajectory length, at the end of which the exploration episode is terminated).


\cite{Chaplot2020semantic} %\bc{Skip semantics ?}
%How should an exploration policy decide which trajectory should be labeled? One possibility is to use a
%trained object detector’s failure cases as an external reward. However,
%this will require labeling millions of frames required for training RL policies, which is infeasible. 
%Instead, we 
explored a self-supervised approach for training our exploration policy by introducing 
semantic curiosity which is based on observation consistency.
%– the detection outputs should be consistent. Therefore, our semantic curiosity  
It rewards trajectories with inconsistent labeling behavior and
encourages the exploration policy to explore such areas. 
%The exploration policy trained via semantic curiosity generalizes to novel scenes and helps
%train an object detector that outperforms baselines trained with other possible alternatives such as random exploration, prediction-error curiosity, and coverage-maximizing exploration.

%------------------------
\cite{Chaplot2021SEAL}
%In this paper, we explore how we can build upon the data and models of Internet images and use them to adapt to robot vision without requiring any extra labels. We present a framework called Self-supervised Embodied Active Learning (SEAL). It utilizes 
trains perception models on internet images to learn an active exploration policy. 
%The observations gathered by this exploration policy are labelled using 3D consistency and used to improve the perception model. We 
They build 3D semantic maps to learn both action and perception models.
%in a completely self-supervised manner. 
These semantic maps are used and to compute an intrinsic motivation reward 
%for training the exploration policy and 
to label
%for labelling 
the observations using spatio-temporal 3D consistency. % and label propagation. 
%We demonstrate that the SEAL framework can be used to close the action-perception loop: it improves object detection and instance segmentation performance of a pretrained perception model by just moving around in training environments and the improved perception model can be used to improve Object Goal Navigation.
%by training perception models on a large collection of internet images  and an active exploration policy for spatio-temporal 3D consistency.

\cite{chaplot21objectgoal}
%This work studies the problem of object goal navigation which involves navigating to an instance of the given object category in unseen environments. End-to-end learning-based navigation methods struggle at this task as they are ineffective at exploration and long-term planning. We propose a modular system called, ‘GoalOriented Semantic Exploration’  which 
builds an episodic semantic map and uses it
to explore the environment efficiently based on the goal object category. 
%Empirical results in visually realistic simulation environments show that the proposed model outperforms a wide range of baselines including end-to-end learning-based methods as well as modular map-based methods and led to the winning entry of the CVPR-2020 Habitat ObjectNav Challenge. Ablation analysis indicates that the proposed model learns semantic priors of the relative arrangement of objects in a scene, and uses them to explore efficiently. Domain-agnostic module design allow us to transfer our model to a mobile robot platform and achieve similar performance for object goal navigation in the real-world.

\cite{Chen19exploration}
%task-driven navigation.
%But, how to effectively explore a new environment to enable a variety of down-stream
%tasks has received much less attention. In this work, we 
study how agents can autonomously explore %realistic and 
complex environments with no %the
special task rewards. %a learning-based approach and
They %investigate different
%policy architectures, reward functions, and training paradigms. 
%Wend that use of 
use policies with spatial memory that are bootstrapped with imitation learning and
finetuned with coverage rewards derived purely from on-board sensors can
be effective at exploring novel environments~\cite{Chen19exploration}
%We show that our learned exploration policies can explore better than classical approaches based on geometry
%alone and generic learning-based exploration techniques. Finally, we also show
%how such task-agnostic exploration can be used for down-stream tasks.


\\
